Constructing Budgeted KGW Evasion through Token-Event Evidence Replacement

KGW watermarks bias sampling to accumulate keyed detection evidence. We construct budgeted evasion through token-event evidence replacement using ordinary phrase rewrites. Our construction jointly selects compositions of LLM-proposed alternatives from an independent model and measures global token-edit distance on complete outputs. At the largest attainable cost within the budget, exact coverage search maximizes removal of original scored token pairs. It uses a known tokenizer without the key, detector feedback or queries to the watermarked model. Exact accounting separates source evidence removed, evidence created and length effects, with initial strength setting the required reduction. Separate signed-event analysis found that mean suppression arose mainly from removing watermark-enriched source events. In controlled, occurrence-counted, one-token-context KGW tests on short passages, 39 of 82 qualified, initially detected sources yielded rewrites with terminal detector score Z < 4 that passed blinded source-relative model review, at a mean actual token-edit cost of 16.0% under a 20% allowance. To examine whether this initial requirement can be inferred, a separate historical 95-passage study estimated initial detector score Z0 from generation traces with correlation 0.793 and an in-sample association beyond length. This aggregate information did not establish improved allocation, and the separate no-trace stopping test did not reliably exploit cheaper reviewed crossings in the candidate bank. Comparisons did not establish an advantage over simpler selection and ordinary constrained rewriting. The construction makes budgeted evidence replacement executable while exposing limits in signed reduction and recognition of sufficient editing.

==> figures/evasion_replacement_table.tex <==
% Exact saved phrase pairs; bold words are a deterministic word diff.
\begingroup\fontsize{9}{10.5}\selectfont
\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.03}
\begin{tabularx}{13.45cm}{@{}>{\centering\arraybackslash}p{0.28cm} >{\raggedright\arraybackslash}X @{\hspace{5pt}$\to$\hspace{5pt}} >{\raggedright\arraybackslash}X@{}}
& \textcolor{foneSource}{\textbf{Original phrase (token positions)}} & \textcolor{foneOutput}{\textbf{Replacement (token positions)}} \\
\midrule
\textbf{1} & \textcolor{foneSource}{1--12: \textbf{After} \textbf{two} weeks \textbf{following} the establishment of a Special Committee tasked with} & \textcolor{foneOutput}{1--11: \textbf{Two} weeks \textbf{after} the establishment of a Special Committee tasked with} \\[3pt]
\textbf{2} & \textcolor{foneSource}{28--39: their comprehensive report \textbf{exposed} \textbf{grave} misconduct that \textbf{deeply} \textbf{disturbed} the democratic process} & \textcolor{foneOutput}{27--38: their comprehensive report \textbf{revealed} \textbf{serious} misconduct that \textbf{profoundly} \textbf{disrupted} the democratic process} \\[3pt]
\textbf{3} & \textcolor{foneSource}{56--71: \textbf{thereby} prompting \textbf{calls} for \textbf{enhanced} regulations to ensure parliamentary conduct \textbf{adheres} \textbf{to} high ethical standards} & \textcolor{foneOutput}{55--69: \textbf{thus} prompting \textbf{demands} for \textbf{stronger} regulations to ensure \textbf{that} parliamentary conduct \textbf{meets} high ethical standards} \\[3pt]
\end{tabularx}
\endgroup


==> figures/evasion_trajectory_data.tex <==
% Exact measured original-CUDA prefix curves; no smoothed/interpolated states.
\def\DemoOriginalCoordinates{(2,1) (3,1.41421356237309) (4,0.577350269189626) (5,1) (6,1.34164078649987) (7,1.63299316185545) (8,1.13389341902768) (9,1.41421356237309) (10,1.66666666666667) (11,1.26491106406735) (12,0.904534033733291) (13,0.577350269189626) (14,0.832050294337844) (15,1.0690449676497) (16,1.29099444873581) (17,1.5) (18,1.69774937525433) (19,1.88561808316413) (20,2.06474160483506) (21,2.23606797749979) (22,2.40039679259592) (23,2.55840859626733) (24,2.71068738274197) (25,2.85773803324704) (26,3) (27,3.13785816221094) (28,3.27165152540788) (29,3.40168025708304) (30,3.52821142536399) (31,3.65148371670111) (32,3.77171134256227) (33,3.88908729652601) (34,4.00378608698105) (35,4.11596604342021) (36,4.22577127364258) (37,4.33333333333333) (38,4.43877265724465) (39,4.54219979166135) (40,4.64371646034753) (41,4.74341649025257) (42,4.84138661854679) (43,4.93770719878694) (44,5.03245282097595) (45,4.82418151324422) (46,4.91934955049954) (47,5.0130265092665) (48,5.10527470242631) (49,4.90747728811182) (50,5) (51,5.09116882454314) (52,5.18103631090364) (53,5.26965186413968) (54,5.35706199399887) (55,5.44331053951817) (56,5.25875892721329) (57,5.34522483824849) (58,5.43058266396668) (59,5.51487018010835) (60,5.59812317217543) (61,5.68037557443754) (62,5.76165959698032) (63,5.84200584200876) (64,5.92144341047789) (65,6) (66,6.07770199487121) (67,6.15457454896664) (68,6.23064166217157) (69,6.30592625094466) (70,6.38045021354577) (71,6.21518876853885) (72,6.28994278842742)}
\def\DemoOriginalEnd{6.28994278842742}
\def\DemoRewrittenCoordinates{(2,-1) (3,-1.41421356237309) (4,-1.73205080756888) (5,-1) (6,-0.447213595499958) (7,-0.816496580927726) (8,-0.377964473009227) (9,0) (10,-0.333333333333333) (11,-0.632455532033676) (12,-0.904534033733291) (13,-0.577350269189626) (14,-0.277350098112615) (15,0) (16,0.258198889747161) (17,0.5) (18,0.727606875108999) (19,0.942809041582063) (20,1.14707866935281) (21,1.34164078649987) (22,1.52752523165195) (23,1.70560573084488) (24,1.87662972651367) (25,2.04124145231932) (26,2.2) (27,2.35339362165821) (28,2.50185116648838) (29,2.64575131106459) (30,2.78543007265578) (31,2.55603860169078) (32,2.33486892634807) (33,2.47487373415292) (34,2.26300952742407) (35,2.40098019199512) (36,2.19740106229414) (37,2.33333333333333) (38,2.46598480958036) (39,2.5955427380922) (40,2.72217861468648) (41,2.84604989415154) (42,2.96730147588352) (43,3.08606699924184) (44,2.89747283631949) (45,3.01511344577764) (46,3.13049516849971) (47,3.24372303540774) (48,3.06316482145579) (49,3.17542648054294) (50,3.28571428571429) (51,3.39411254969543) (52,3.50070021007002) (53,3.60555127546399) (54,3.7087352266146) (55,3.53815185068681) (56,3.64067925730151) (57,3.74165738677394) (58,3.84114383548863) (59,3.93919298579168) (60,4.03585624040554) (61,4.13118223595458) (62,4.22521703778557) (63,4.0640040640061) (64,3.90563288776201) (65,4) (66,3.84507677226546) (67,3.93892771133865) (68,4.03159166375807) (69,3.88057000058133) (70,3.97273315183038)}
\def\DemoRewrittenEnd{3.97273315183038}
\def\DemoOriginalRegions{1/12/1,28/39/2,56/71/3}
\def\DemoRewrittenRegions{1/11/1,27/38/2,55/69/3}
\def\DemoRegionWindows{1/12/1,27/39/2,55/71/3}


==> figures/figure_one_data.tex <==
% Generated from unchanged frozen weighted-p20 manuscript witnesses.
\def\FigOneEscapeADRaw{8.5}
\def\FigOneEscapeAD{8.500}
\def\FigOneEscapeCreatedRaw{1.5}
\def\FigOneEscapeCreated{+1.500}
\def\FigOneEscapeBoundaryRaw{-0.239051820516568}
\def\FigOneEscapeBoundary{-0.239}
\def\FigOneEscapeGainRaw{9.76094817948343}
\def\FigOneEscapeGain{9.761}
\def\FigOneEscapeHeadroomRaw{9.64770045364728}
\def\FigOneEscapeHeadroom{9.648}
\def\FigOneEscapeSourceZ{6.290}
\def\FigOneEscapeFinalZ{3.973}
\def\FigOneEscapeCost{14}
\def\FigOneEscapeTokens{72}
\def\FigOneEscapeDestroyed{21}
\def\FigOneDetectedADRaw{6}
\def\FigOneDetectedAD{6.000}
\def\FigOneDetectedCreatedRaw{-3}
\def\FigOneDetectedCreated{-3.000}
\def\FigOneDetectedBoundaryRaw{-0.350833588182592}
\def\FigOneDetectedBoundary{-0.351}
\def\FigOneDetectedGainRaw{2.64916641181741}
\def\FigOneDetectedGain{2.649}
\def\FigOneDetectedHeadroomRaw{10.0217494138479}
\def\FigOneDetectedHeadroom{10.022}
\def\FigOneDetectedSourceZ{5.745}
\def\FigOneDetectedFinalZ{5.303}
\def\FigOneDetectedCost{21}
\def\FigOneDetectedTokens{133}
\def\FigOneDetectedDestroyed{32}


==> figures/figure_one_outcome.tex <==
% Complete-output accounting: remaining margin, not sequential edit scores.
\begingroup
\input{figures/figure_one_styles}
\input{figures/figure_one_data}
\edef\side{\FigOneRole}
\pgfmathsetmacro{\ad}{\csname FigOne\side ADRaw\endcsname}
\pgfmathsetmacro{\created}{\csname FigOne\side CreatedRaw\endcsname}
\pgfmathsetmacro{\boundary}{\csname FigOne\side BoundaryRaw\endcsname}
\pgfmathsetmacro{\head}{\csname FigOne\side HeadroomRaw\endcsname}
\pgfmathsetmacro{\afterSource}{\head-\ad}
\pgfmathsetmacro{\afterCreated}{\afterSource-\created}
\pgfmathsetmacro{\remaining}{\afterCreated-\boundary}
\begin{tikzpicture}[x=1cm,y=1cm,font=\fontsize{9}{10.5}\selectfont,
  every node/.style={inner sep=1pt,text=foneInk}]
\path[use as bounding box] (0,-0.2) rectangle (6.5,4.9);
\node[anchor=west,font=\fontsize{10}{11}\selectfont\bfseries] at (0.1,4.65)
  {$Z:\csname FigOne\side SourceZ\endcsname
    \to\csname FigOne\side FinalZ\endcsname$};
\node[anchor=west] at (0.1,4.25)
  {$q=\csname FigOne\side Cost\endcsname$ of
   $N=\csname FigOne\side Tokens\endcsname$ tokens;
   $D=\csname FigOne\side Destroyed\endcsname$ events};
% Shared margin domain [-1,11], with no magnification near zero.
\node[rotate=90] at (0.14,2.35) {Remaining margin};
\begin{scope}[shift={(0.7,0.95)},y=0.26cm]
  \foreach \v in {0,5,10}{
    \draw[foneGray!25,line width=0.3pt] (0,\v)--(5.7,\v);
    \node[anchor=east] at (-0.08,\v) {\v};
  }
  \draw[foneInk,dashed,line width=0.6pt] (0,0)--(5.7,0);
  \draw[foneGray!70,line width=0.4pt] (0,-1)--(0,11);
  \path[fill=foneGray!35] (0.25,0) rectangle (0.75,\head);
  \path[fill=foneSource] (1.4,\head) rectangle (1.9,\afterSource);
  \path[fill=foneOutput] (2.55,\afterSource) rectangle (3.05,\afterCreated);
  \path[fill=foneGray] (3.7,\afterCreated) rectangle (4.2,\remaining);
  \path[fill=foneInk] (4.85,0) rectangle (5.35,\remaining);
  \foreach \a/\b/\v in {0.75/1.4/\head,1.9/2.55/\afterSource,
                         3.05/3.7/\afterCreated,4.2/4.85/\remaining}{
    \draw[foneGray!65,densely dotted] (\a,\v)--(\b,\v);
  }
  \node[anchor=south] at (0.5,{\head+0.2})
    {\pgfmathprintnumber[fixed,precision=3]{\head}};
  \node[anchor=south] at (1.65,{\head+0.2})
    {$-\pgfmathprintnumber[fixed,precision=3]{\ad}$};
  \pgfmathsetmacro{\createdChange}{-\created}
  \pgfmathsetmacro{\lengthChange}{-\boundary}
  \node[anchor=south] at (2.8,{max(\afterSource,\afterCreated)+0.2})
    {$\pgfmathprintnumber[fixed,precision=3,showpos]{\createdChange}$};
  \node[anchor=south] at (3.95,{max(\afterCreated,\remaining)+0.2})
    {$\pgfmathprintnumber[fixed,precision=3,showpos]{\lengthChange}$};
  \node[anchor=south,font=\fontsize{9}{10.5}\selectfont\bfseries]
    at (5.1,{max(0,\remaining)+0.2})
    {$\pgfmathprintnumber[fixed,precision=3,showpos]{\remaining}$};
\end{scope}
\foreach \x/\label in {1.2/Initial,2.35/{Source\\loss},
                        3.5/{New\\states},4.65/Length,5.8/Final}{
  \node[anchor=north,align=center] at (\x,0.52) {\label};
}
\end{tikzpicture}
\endgroup


==> figures/figure_one_trajectory.tex <==
\begingroup
\input{figures/figure_one_styles}
\input{figures/evasion_trajectory_data}
\begin{tikzpicture}[x=0.12cm,y=0.40cm,
  font=\fontsize{9}{10.5}\selectfont,
  every node/.style={inner sep=0pt,text=foneInk}]
\path[use as bounding box] (-9,-6.1) rectangle (92,8.45);
% Gray windows group each pair of source/output phrase intervals. Exact
% one-based token ranges are shown separately in the Src/Out strips below.
\foreach \a/\b/\id in \DemoRegionWindows{
  \fill[foneGray!8] ({\a-0.5},-2.2) rectangle ({\b+0.5},7.0);
}
\foreach \z in {-2,0,2,6}{
  \draw[foneGray!15,line width=0.3pt] (0,\z)--(75,\z);
}
\foreach \n in {20,40,60}{
  \draw[foneGray!15,line width=0.3pt] (\n,-2.2)--(\n,7.0);
}
\draw[foneInk,line width=0.5pt] (0,-2.2)--(75,-2.2);
\draw[foneInk,line width=0.5pt] (0,-2.2)--(0,7.0);
\foreach \n in {0,20,40,60,72}{
  \draw[foneInk] (\n,-2.2)--(\n,-2.45);
  \node[anchor=north] at (\n,-2.75) {\n};
}
\foreach \z in {-2,0,2,4,6}{
  \draw[foneInk] (0,\z)--(-1,\z);
  \node[anchor=east] at (-1.7,\z) {\z};
}
\node[rotate=90] at (-7.2,2.4) {Cumulative KGW score $Z_t$};
\node at (36,-3.85) {Token-prefix length $n$; scored events $t=n-1$};
\draw[foneInk,dashed,line width=0.8pt] (0,4)--(75,4);
\draw[foneSource,line width=1.0pt] plot coordinates {\DemoOriginalCoordinates};
\draw[foneOutput,line width=1.15pt,dash pattern=on 3pt off 1.3pt]
  plot coordinates {\DemoRewrittenCoordinates};
\foreach \a/\b/\id in \DemoRegionWindows{
  \node[circle,draw=foneGray!65,fill=white,minimum size=3.4mm,
    font=\fontsize{9}{10}\selectfont\bfseries] at ({(\a+\b)/2},-1.55) {\id};
}
\node[circle,fill=foneSource,minimum size=4pt] at (72,\DemoOriginalEnd) {};
\node[diamond,fill=foneOutput,minimum size=5pt] at (70,\DemoRewrittenEnd) {};
\node[anchor=west,text=foneSource] at (76,6.55) {$Z_0=6.290$};
\node[anchor=west,text=foneOutput] at (76,3.25) {$Z'=3.973$};
% Dedicated legend row outside the plotting rectangle.
\draw[foneSource,line width=1pt] (1,7.85)--(6,7.85);
\node[anchor=west] at (8,7.85) {Original source};
\draw[foneOutput,line width=1.15pt,dash pattern=on 3pt off 1.3pt]
  (32,7.85)--(37,7.85);
\node[anchor=west] at (39,7.85) {Selected rewrite};
\draw[foneInk,dashed,line width=0.8pt] (67,7.85)--(72,7.85);
\node[anchor=west] at (74,7.85) {Threshold $4$};
\node[anchor=east,text=foneSource] at (-1.7,-4.75) {Src};
\node[anchor=east,text=foneOutput] at (-1.7,-5.55) {Out};
\foreach \a/\b/\id in \DemoOriginalRegions{
  \draw[foneSource,line width=2.8pt] ({\a-0.5},-4.75)--({\b+0.5},-4.75);
  \foreach \n in {\a,\b}{
    \draw[foneSource,line width=0.5pt] (\n,-4.52)--(\n,-4.98);
  }
}
\foreach \a/\b/\id in \DemoRewrittenRegions{
  \draw[foneOutput,line width=2.8pt] ({\a-0.5},-5.55)--({\b+0.5},-5.55);
  \foreach \n in {\a,\b}{
    \draw[foneOutput,line width=0.5pt] (\n,-5.32)--(\n,-5.78);
  }
}
\end{tikzpicture}
\endgroup

